Basic Set Theory and Algebra: Hints on Representation, Topology, Geometry, Analysis

In these self-contained low prerequisite introductory notes we first present (in part 1) basic concepts of set theory and algebra without explicit category theory. We then present (in part 2) basic category theory involving a somewhat detailed discussion of system limits and the exact imbedding of abelian categories. This is followed (in part 3) by a discussion of localization, homological algebra, and generalizations of additive and abelian categories such as triangulated and derived categories. Based on the concepts of category theory from parts 2 and 3, (in part 4) we provide hints for constructive discussions on familiar mathematics such as representation theory and topological geometry/analysis (i.e., topology-based geometry/analysis). If events permit, the notes will be revised/updated regularly.

==> parts/front/Frontmatter.tex <==
\newpage
%%###########################################################################################################
\subsection*{Copy Right Notice}
%%###########################################################################################################
These notes may be used in any form (including edited/modified forms) by an individual to jump-start or improve their studies. The notes may not be used for propaganda or commercial purposes.

\newpage
%%###########################################################################################################
\subsection*{Dedication}
%%###########################################################################################################
To my caring father, Barnabas Ngocho, and to my caring teacher, Samson Bamgah, both of whose inspiring passion for knowledge and transcendental instructions, even in the hands of a helpless lamb, have challenged and outlived possibly the worst of deliberate(ly systemized) injustice. Unlike most, these gallant champions of virtue never lied to me about the undesired that existed in place of the desired. Without their early warning I would have died a long time ago just from the shock of surprise alone. Their daring spirits supplied the following \ul{Armor of The Lamb}, which not-so-simply refers respectively to patience/compassion, courage/bravery, endurance/perseverance.

{\flushleft \ul{Armor of The Lamb}:} To rest in the wind in silent hope. Lonesome but fearless. To ride the winds.

{\flushleft \ul{The advice in summary}:} Almost everyone believes impeccably that you can't make it, but I know you can do a lot more than simply make it, as long as you can find a way to ignore/avoid their careless presumptions in favor of logical deductions.

\newpage
%%###########################################################################################################
\subsection*{Acknowledgements}
%%###########################################################################################################
I am grateful to all instructors whose classes I attended at Syracuse University. I am equally grateful for the efforts of all selfless persons who try to share (especially on the internet in various ways) the little they have, even when it seems hopelessly insignificant compared to what others appear to possess. Without such brave persons, I never would have been able to learn much, let alone find something to write down.

\newpage
\subsection*{Abstract}
In these minimal prerequisite introductory notes, we first present basic concepts of set theory and algebra without explicit category theory. We then present basic category theory involving a detailed discussion of abelian categories, homological algebra and (exact) imbedding of abelian categories into module categories, and some generalizations of abelian categories such as triangulated and derived categories. Based on the concepts of category theory, we provide some hints for constructive discussions of familiar mathematics such as topological geometry and measure theoretic analysis. If events permit, the last part of the notes will be extended in time.


%%###########################################################################################################
\tableofcontents
%%###########################################################################################################

\chapter{Description of Contents}
\section{Motive and objective}
Those who try to listen/read but fail to understand (for whatever reasons) are often wrongly considered to be stupid. However, the only truly stupid persons are those that have ears/literacy (and of course the chance, health, ...) and yet refuse to listen/read in favor of presumption (i.e., the attractive comfort therein). Moreover, in any situation where those who don't listen are indeed stupid, those who don't read are even stupider, because truth is a lot more easily written down than spoken out.

These are merely personal notes of the writer on some basic aspects of (algebra-oriented) mathematics, and not a specialized textbook on any particular area of the vast subject of mathematics. While a ``graduate student'' at Syracuse University from 2015-2020, the writer took notes as carefully as he could during several mathematics course lectures given by various instructors at different times. As usual, these lecture notes contained interesting ideas/outlines (footnote\footnote{The missing details were often about results from set theory and category theory, which are central areas of mathematics that nevertheless are (for yet mysterious reasons) often either only briefly mentioned in depending courses or ignored altogether.}) for the somewhat tedious proofs of certain well-known standard results in algebra, examples of which are K\"unneth formulas. Since the writer was more interested in the proof details than in the results themselves or their uses, he decided afterwards to undertake the challenge of efficiently reconstructing the omitted connections that help explain such intriguing results.

The notes should be structurally self-contained and therefore best for personal study but, of course, (along with needed supplements/exercises) can also be easily used to teach a course. The notes assume nothing beyond high school mathematics/logic along with a certain degree of maturity and, of course, the willingness to think/reason in a flexible manner towards intelligent abstraction (footnote\footnote{Here, ``\emph{abstraction}'', which is essentially ``\emph{Compressed/efficient generalization via symbolic, rather than concrete, representation.}'' is done in a carefully guided way, so that it is not merely ``\emph{nonsense}''.}).

The notes present algebra concepts, hopefully, in a ``purified'' manner in the sense that they avoid (as much as possible) equally important but often distractive/uncertain details such as historical accounts, award of credit, credibility of sources, applicability, and more. The notes are intended to be an efficient attempt to reveal what the writer believes makes algebra work (or lies at the heart of algebra), notably, the roles of set theory and category theory, but neither who is credited for what piece of algebra, nor what algebra can do. Therefore, the notes are best for persons who by nature like/enjoy doing or sharing mathematics even on their own (i.e., even with little or no appreciation/encouragement/support from others).

Recognize however that it is only through application (e.g., working on exercises from mathematics texts/literature) that one can really begin to appreciate the strength/significance of these fundamentals. The emphasis here (quite contrary to common practice) is on first getting a fairly extensive framework of the fundamentals before attempting to apply/evaluate them. That is, the ``motto'' is to ``get the idea first'' (which is by no means a trivial task, and so might require patience/endurance depending on natural ability), and then skillful/enjoyable exercise is likely to follow afterwards.

\ul{Important note}: Names of persons, and all references, are used strictly as reasonably convenient guiding labels (for easily/efficiently navigating through the literature), and no crediting whatsoever is implied, understood, or even recognized by the writer. To the writer, a relevant/important/great person is simply someone who is willingly doing their very best in whatever situation they happen to find themselves (irrespective of whether or not any of their efforts are ever going to be appreciated). This is called justice.

\section{About errors and revision}
To any civil person, an error is never a crime, unless you have committed it intentionally or out of carelessness. Nevertheless, errors are undesirable, even though they are far more harmless than (for example) the famous blind suicide mission known as politics. This is rather ironic since we (at least those of us who value learning) learn mostly through errors, both ours and those of others.

These notes have no deliberate/intentional errors, but they might have things that can easily be misunderstood/misinterpreted by readers and so become real errors. In that case, feel free to silently create an improved version of the notes for yourself. If circumstances permit, the notes will be revised/updated regularly.

\section{Scientific setting}
The \emph{nature} of a thing (physical \emph{object} or \emph{system}) refers to those aspects (properties) of it that do not depend on any particular/individual viewpoint on (observation of) it. \emph{Science} is an attempt to find the nature of a thing by putting together various viewpoints (perceptions) of it, including its compositions in terms of smaller things (e.g., its structural \emph{appearances}), its roles as part of larger things (e.g., its \emph{origins}), its effects through interaction with other things (i.e., its \emph{environment}), etc.

\emph{Mathematics} is a simplified/\emph{mechanical} language (means of description/communication) of science. It consists roughly (i.e., after ignoring overlap) of three major parts: \emph{analysis} (object \emph{size} measurements), \emph{geometry} (object \emph{shape} classifications), \emph{algebra} (object background/\emph{reference}/framework categorizations).

\emph{Statistics} is a method of scientific investigation that involves the learning of \emph{characteristics} of a \emph{population} (a system of objects) from \emph{data} collected through a \emph{study} on a \emph{sample} (an accessible portion) of the population. \emph{Probability} (a field of analysis) is a mathematical tool for avoiding \emph{biased samples} (samples that do not sufficiently represent the population) in statistics.

In these notes, our main concern is not with any specific area or application of \emph{mathematical science}, but rather with some basic concepts that underly advanced studies in (algebra-oriented) mathematics. The basic idea is to unhide/expose the ingredient that makes mathematics outstanding as an instructional tool. This ingredient is in the form of a genuine \ul{attempt} to reveal as much of the truth about nature as possible through mathematical rigor. At every step, we \ul{attempt} to build an \emph{unambiguous} conceptual foundation based on which certain results can then be \emph{unambiguously} established. %(footnote\footnote{Of course, one has to understand what nature is really, but the lack of a definition for nature is nowhere nearly as criminal as the arrogance of the spineless mental tower of Babel known as politics.}).

\section{Organization}
The notes are divided into three main parts. Part I swiftly, but efficiently, introduces set theory and algebra concepts without explicit category theory. Also introduced right from the beginning of Part I is the concept of (proper) classes, a generalization of sets, which serves as an indication that there are equally useful objects/structures beyond set-based objects/structures such as groups, rings, modules, algebras, topological spaces, etc. These other useful objects/structures include (class-based) graphs, categories, systems, functors, etc.

Part II introduces basic category theory along with commonly used descriptive tools such as diagrams, limits, localization, etc. Because of their central role, abelian categories, along with their homological algebra and (exact) imbedding into module categories are discussed extensively. Some generalizations of abelian categories such as triangulated and derived categories are also discussed.

Part III is mostly application-oriented. Some chapters in this part provide hints for constructive (e.g., categorical) discussions of familiar (Part I)-based mathematics with the help of the ideas/methods introduced in Part II. Notable among the main application areas considered in Part III are topology/geometry and measure theory/analysis. In the discussion in Part III, \emph{algebra} (Parts I and II) is used to introduce \emph{topology/geometry}, which is in turn used to introduce \emph{measure theory/analysis}. Note however that some of the subsequent/\ul{pending} applications in Part III (after geometry and analysis) might be directly based on Parts I and II, possibly without the involvement of topology or measure theory.

%%###########################################################################################################
\section{Prerequisite}
%%###########################################################################################################
As already mentioned in ``motive and objective'', the notes are (i) structurally self-contained and (ii) assume nothing beyond high school mathematics/logic along with a certain degree of maturity and a willingness to be flexible with abstraction. Some college or graduate level mathematics might be helpful, but the notes are designed with the assumption that the reader has no streamlined previous knowledge. Therefore, it is recommendable for a reader with prior knowledge to attempt to view these notes as a cleaned up review/update of their knowledge.

%%###########################################################################################################
\subsection*{Notation and conventions}
%%###########################################################################################################
Our preferred set containment operations are $\subset$ for non-strict containment, and $\subsetneq$ for strict containment. However, when dealing with a partially ordered set (poset), we will for convenience also use $\subseteq$ (in place of $\subset$) for non-strict containment. That is $\subset,\subseteq$ will each denote ``non-strict containment'' while $\subsetneq$ will denote ``strict containment''.

Capital letters such as $A,B,\cdots$ will denote sets (and later, objects in a category and functors between categories), meanwhile "curly" capital letters such as $\A,\B,\cdots$ will denote collections/families of sets (and later, categories). Lower case letters will denote elements of a set, i.e., an arbitrary element of a set $A$ is denoted by $a\in A$ (and later, morphisms in a category). If $f:X\ra Y$, $x\mapsto f(x)$ is a \emph{mapping} of sets (i.e., a rule that assigns to each element $x\in X$ a \emph{unique} element $f(x)\in Y$), then the value of $f$ at $x\in X$ is denoted by $f(x)$ or $f_x$ or $f^x$, depending on convenience. The same notation applies to indexed collections. For example, we can write $\{C(\al)\}_{\al\in A}$ or $\C=\{C_\al\}_{\al\in A}$ or $\C=\{C^\al\}_{\al\in A}$. For countable collections, we will often write $\C=\{A_i\}_{i\in C}$, for a countable set $C$. That is, we mostly (but not always) use $\al,\beta,\gamma,\cdots$ for arbitrary indices and mostly (but not always) use $i,j,k,l,\cdots$ for countable indices. In cases where the countable set $C\subset\Integer$, we will often (but not always) use $m,n,r,s,t,\cdots$, e.g., $\C=\{A_n\}_{n=1}^\infty$.

Any specialized notation/convention that deviates from the above basic rules will be explicitly stated (along with any associated terminology) in definitions. Such specialized notation is common in all chapters/sections. Note that all chapters/sections adopt and use notation introduced in ``earlier'' chapters/sections, often without any explicit reminder.

We will sometimes abbreviate certain frequent phrases as follows.  \ul{~$\exists$~} stands for \ul{``there exists''}. \ul{~$\nexists$~} stands for \ul{``there does not exist''}. \ul{~$\exists!$~} stands for \ul{``there exists a unique''}. \ul{~$:=$~} stands for \ul{``defined to be''}. \ul{~$\Ra$~} stands for \ul{``implies''}. \ul{\emph{iff} (or $\iff$)} stands for \ul{``if and only if''}. \ul{\emph{s.t.}} or \ul{~$:$~} stands for \ul{``such that''}. \ul{~$|$~} stands for \ul{``restricted to''}. \ul{\emph{a.e.}} stands for \ul{``almost everywhere''}. \ul{\emph{a.e.f.}} stands for \ul{``all except finitely many''}. \ul{\emph{wlog}} stands for \ul{``without loss of generality''}. \ul{\emph{nbd}} stands for \ul{``neighborhood''}. \ul{\emph{resp.}} stands for \ul{``respectively''}. \ul{\emph{equiv.}} stands for \ul{``equivalently''}. \ul{\emph{const.}} stands for \ul{``constant''}. \ul{~$\ll$~} stands for \ul{``much less than''}. \ul{~$\gg$~} stands for \ul{``much greater than''}.

The symbol $\cong$ will denote \ul{``isomorphism''} (of all types of objects), the symbol $\sim$ (among others) will denote an \ul{``equivalence relation''}, the symbol $\simeq$ (among others) will denote \ul{``equivalence of objects''} (e.g., chain complexes/morphisms) in a category, and the symbol $\approx$ will denote \ul{``cardinal equivalence''} of classes of objects. 





